LAPP: Large Language Model Feedback for Preference-Driven Reinforcement Learning

We introduce Large Language Model-Assisted Preference Prediction (LAPP), a novel framework for robot learning that enables efficient, customizable, and expressive behavior acquisition with minimum human effort. Unlike prior approaches that rely heavily on reward engineering, human demonstrations, motion capture, or expensive pairwise preference labels, LAPP leverages large language models (LLMs) to automatically generate preference labels from raw state-action trajectories collected during reinforcement learning (RL). These labels are used to train an online preference predictor, which in turn guides the policy optimization process toward satisfying high-level behavioral specifications provided by humans. Our key technical contribution is the integration of LLMs into the RL feedback loop through trajectory-level preference prediction, enabling robots to acquire complex skills including subtle control over gait patterns and rhythmic timing. We evaluate LAPP on a diverse set of quadruped locomotion and dexterous manipulation tasks and show that it achieves efficient learning, higher final performance, faster adaptation, and precise control of high-level behaviors. Notably, LAPP enables robots to master highly dynamic and expressive tasks such as quadruped backflips, which remain out of reach for standard LLM-generated or handcrafted rewards. Our results highlight LAPP as a promising direction for scalable preference-driven robot learning.

==> algorithms/two_algorithms.tex <==
\begin{figure}[t]  % or [H] if using float package
\centering
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\footnotesize
\caption{\textsc{LAPP} \textnormal{- Preference Predictor Training}}\label{alg:lapp_preference_predictor_training}
\textbf{Require:} Ensemble of preference predictors $\{\hat{r}_i\}$, preference predictor training dataset $D_p$\\
\textbf{Hyperparameters:} Minimum iteration $N_{min}$, Maximum iteration $N_{max}$, pool of predictors number $M$, selected predictors number $C$, overfitting scale $\alpha$, LLM feedback error rate $\epsilon$.\\
\textcolor{pinkyred}{//Split into training and validation sets} \\
$D_p^{train}, D_p^{val} \leftarrow split(D_p)$ \\
$val\_loss\_list \leftarrow \left[\ \right]$\\
\For{$M$ predictors}{
Randomly initialize $\hat{r}_i$\\
\For{$m \leftarrow 0$ \KwTo $N_{max}-1$ epochs}{
\textcolor{pinkyred}{// Sample from $D_p^{train}$} \\
$(s_t^{train}, a_t^{train}) \sim D_p^{train}$ \\
\textcolor{pinkyred}{// Predict preference reward}\\
$r_t^{train} = \hat{r}_i(s_t^{train}, a_t^{train})$ \\
\textcolor{pinkyred}{// Train the preference predictor}\\
Calculate loss $\mathcal{L}^{CE}_{train}(r_t^{train})$ with Equation \ref{eq:adjusted_ce_loss} \\
% Update $\hat{r}_i$ with $\mathcal{L}^{CE}_{train}(r_t^{train})$ \\
$\hat{r}_i \leftarrow \mathrm{Adam}\Bigl(\hat{r}_i,\nabla_{\hat{r}_i}\mathcal{L}^{CE}_{train}(r_t^{train})\Bigr)$ \\
\textcolor{pinkyred}{// Sample from $D_p^{val}$} \\
$(s_t^{val}, a_t^{val}) \sim D_p^{val}$ \\
\textcolor{pinkyred}{// Predict preference reward}\\
$r_t^{val} = \hat{r}_i(s_t^{val}, a_t^{val})$ \\
Calculate loss $\mathcal{L}^{CE}_{val}(r_t^{val})$ with Equation \ref{eq:adjusted_ce_loss} \\
\If{$\mathcal{L}^{CE}_{val}(r_t^{val}) > \alpha \cdot \mathcal{L}^{CE}_{train}(r_t^{train})\ \textbf{and}\ n>N_{min}$}{
val\_loss\_list.append ($\mathcal{L}^{CE}_{val}(r_t^{val})$) \\
continue;
}
\If{$m == N_{max}-1$}
{val\_loss\_list.append ($\mathcal{L}^{CE}_{val}(r_t^{val})$) \\}
}
}
\textcolor{pinkyred}{// Select the C predictors with smallest validation losses} \\
\(\hat{r}_{i_1}, \hat{r}_{i_2}, ... , \hat{r}_{i_C} \leftarrow \arg\min_{\hat{r}_i \in \{\hat{r}_1,\dots,\hat{r}_M\}}^{C} val\_loss\_list[i]\) \\
\textcolor{pinkyred}{// Use the mean value of the selected predictors as the final predictor} \\
$\hat{r} = mean\left(\hat{r}_{i_1}, \hat{r}_{i_2}, ... , \hat{r}_{i_C}\right)$\\
\Return{$\hat{r}$}
\end{algorithm}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\footnotesize
\caption{\textsc{LAPP}}\label{alg:lapp}
\textbf{Require:} Robot behavior prompt $prompt$, preference generator LLM  $LLM$, environment $E$, policy $\pi$, preference predictor $\hat{r}$, preference predictor training dataset $D_p$, preference data buffer $B_p$ \\
\textbf{Hyperparameters:} Policy optimization epoch number $N$, preference predictors update interval epoch number $M$, per epoch trajectories pairs collection number $K$, per epoch rollouts number $S$, steps in each epoch $T$, preference reward scale $\beta$ \\
\textbf{Initialization:} Randomly initialize $\pi$, $\hat{r}$. $D_p \leftarrow \{ \text{zeros triple}_i \}_{i=1}^{|D_p|}$, $B_p \leftarrow \{ \text{zeros triple}_i \}_{i=1}^{M * K}$.\\
\textcolor{pinkyred}{// Collect initial preference dataset}\\
Rollout $\pi$ and sample $|D_p|$ trajectories pairs $\{ (\sigma^0_i, \sigma^1_i )\}^{|D_p|}_{i=1}$.\\
$\{y_i\}^{|D_p|}_{i=1} \sim \text{LLM}\left(\{ \sigma^0_i, \sigma^1_i \}^{|D_p|}_{i=1},\ prompt\right)$ \\
$D_p \leftarrow \{ (\sigma^0_i, \sigma^1_i, y_i) \}^{|D_p|}_{i=1}$\\
Update $\hat{r}$ with Algorithm \ref{alg:lapp_preference_predictor_training}.\\

$obs \sim E.reset()$ \textcolor{pinkyred}{// reset $E$, get initial observation} \\
\For{$i \leftarrow 0$ \KwTo $N-1$ epochs}{
\textcolor{pinkyred}{ //rollout $\pi$ in $E$ \\}
\For{ $T$ steps}{
$a \sim \pi(obs)$ \ \textcolor{pinkyred}{// sample action from policy}\\
$r_E \sim E(obs)$ \ \textcolor{pinkyred}{// get environment reward $r_E$}\\
$r_p \sim \hat{r}(obs)$ \ \textcolor{pinkyred}{// predict preference reward $r_p$}\\
$r = \beta \cdot r_p + r_E$ \ \textcolor{pinkyred}{// calculate weighted sum}\\
}
Update $\pi$ with PPO algorithm \citep{schulman2017proximal}\\
\textcolor{pinkyred}{// Sample $K$ pairs from $S$ rollouts} \\
$\{ (\sigma^0_k, \sigma^1_k) \}^{K}_{k=1} \sim \{ \sigma_s \}^{S}_{s=1}$ \\
\textcolor{pinkyred}{// Push into the preference data buffer} \\
Push $\{ (\sigma^0_k, \sigma^1_k, None) \}^{K}_{k=1}$ into $B_p$\\
\textcolor{pinkyred}{// Update the preference dataset \\}
\If{(i+1) \% M == 0}{
\textcolor{pinkyred}{// Generate preference labels} \\
$\{y_k\}^{M*K}_{k=1} \sim \text{LLM}\left(\{ (\sigma^0_k, \sigma^1_k) \}^{M*K}_{k=1},\ prompt\right)$ \\
\textcolor{pinkyred}{// Place preference labels into the buffer} \\
$B_p \leftarrow \{ (\sigma^0_k, \sigma^1_k, y_i) \}^{M*K}_{k=1}$ \\
\textcolor{pinkyred}{// Update preference dataset} \\
$D_p \leftarrow \{ \text{triple}_k | \text{triple}_k \in D_p \}^{|D_p|}_{k={M*K+1}} \cup B_p$\\
\textcolor{pinkyred}{// Update preference predictor} \\
Update $\hat{r}$ with Algorithm \ref{alg:lapp_preference_predictor_training}.\\
$B_p \leftarrow \{\}$\\
}
}
\Return{$\pi$}
\end{algorithm}
\end{minipage}
\end{figure}

